Thermodynamic geometry of ideal quantum gases: a general framework and a geometric picture of BEC-enhanced heat engines

Thermodynamic geometry provides a physically transparent framework to describe thermodynamic processes in meso- and micro-scale systems that are driven by slow variations of external control parameters. Focusing on periodic driving for thermal machines, we extend this framework to ideal quantum gases. To this end, we show that the standard approach of equilibrium physics, where a grand-canonical ensemble is used to model a canonical one by fixing the mean particle number through the chemical potential, can be extended to the slow driving regime in a thermodynamically consistent way. As a key application of our theory, we use a Lindblad-type quantum master equation to work out a dynamical model of a quantum many-body engine using a harmonically trapped Bose gas. Our results provide a geometric picture of the BEC-induced power enhancement that was previously predicted for this type of engine on the basis of an endoreversible model [New J. Phys. 24, 025001 (2022)]. Using an earlier derived universal trade-off relation between power and efficiency as a benchmark, we further show that the Bose-gas engine can deliver significantly more power at given efficiency than an equally large collection of single-body engines. Our work paves the way for a more general thermodynamic framework that makes it possible to systematically assess the impact of quantum many-body effects on the performance of thermal machines.

==> Discussion.tex <==
Whether enhanced or diminished work fluctuations result from collective effects, whose nature may be captured under this framework. Since our formalism is originally derived from grand-canonical ensemble, we expect that fluctuations in work output will be drastically enhanced around the critical temperature,resulting from the large density fluctuations, predicted and observed for BECs under a grand-



\subsection{Concluding remarks and outlook}
In this work we have constructed a dynamical framework in which it is possible to describe thermodynamic cycles in the adiabatic response regime for driven quantum gases. Constrained periodic tuning of the chemical potential, under the condition that the average number of particles in the system is fixed, returns an effectively canonical description from a grand-canonical one. This remains thermodynamically consistent in this slow driving limit and provides a systematic approach to determining the adiabatic response coefficients that appear in the slow driving expansion of the thermodynamic forces. Previously established geometric expressions for the work output and dissipation of periodically driven microscopic heat engines can therefore be calculated for such many-body working systems. 

Applying our framework to a harmonically trapped Bose gas under the operation of a Stirling cycle, we calculate the Berry curvature, associated with the quasi-static work output and thermodynamic length, associated with the bound on dissipation for cycles driven in finite time. Our result for the geometric work output confirm what has been recently shown for an endoreversible Otto cycle operating with the same working system, that quasi-static cycles operating across the transition line exhibit an enhanced work output, resulting from the collective nature of a BEC. A new insight into Stirling cycles that operate in finite time, shows that the minimum dissipation incurred in cycles with a boosted work output is also enhanced. Nonetheless, applying these results to a previously established geometric tradeoff relation between the power output and efficiency, indicates that an enhanced power output at a given efficiency is achievable, owing to the collective nature of the working system. This example illustrates the application of our framework in analysing slowly driven cycles of many-body thermal machines. Future studies may apply this framework to investigate other devices to determine the role collective effects play on impacting performance. 


%Whether there are many-body systems whose collective effects may enhance or suppress the performance of the small-scale thermal machines remains an interesting topic of research. 
In the adiabatic response regime, geometric bounds between on work fluctuations and performance have been described for single-body thermal machines \cite{Miller2020}. An open question is whether enhanced or diminished work fluctuations result from collective effects, whose nature may be captured under this framework. Since our formalism is originally derived from grand-canonical ensemble, we expect that fluctuations in work output will be drastically enhanced around the critical temperature,resulting from the large density fluctuations, predicted and observed for BECs under a grand-canonical treatment \cite{Schmitt2014,Crisanti2019}. A curious extension to our framework would be the inclusion of inter-particle interactions. It therefore remains an open question as to how the observed enhanced performance of a Bose gas is influenced by introducing weak interactions between its constituents.

To illustrate the usefulness of this framework we have considered a BEC Stirling cycle


In this work we have developed a dynamical framework which caters for the analysis of engine cycles for a driven quantum gas through the lens of  thermodynamic geometry. Upon fixing the chemical potential such that the average number number of particles within the system remains constant, we have derived a new set of effective adiabatic-response coefficients, which give an effectively canonical description of a working system from the initial grand-canonical picture. The usefulness of this framework has been illustrated by calculating the Berry curvature and thermodynamic length for a BEC Stirling cycle. Here, we have been able to emphasise the collectively enhanced nature of this quantum many-body working system by showing that the quasi-static work output exhibits a boost for cycles that cross the transition. Additionally, our framework has allowed us to explore the bound on dissipation, occurring in slow finite-time cycles. We have shown that this bound, characterized by the thermodynamic length and saturated under optimal parameterization, exhibits an enhancement for the same cycles. Comparing our results with the pre-established power-efficiency trade-off relation \cite{Brandner2020} we have quantitatively shown that the collective effects of the BEC working system lead to a larger power output at a given efficiency than a collection of similar single-body engines.



Owing to the universality of thermodynamic geometry, one could analyze whether different working systems exhibit a similar improvement in performance, by calculating the figure of merit that characterizes the trade-off, under this framework. 

Other bounds on few-body engines that rely on this geometric framework could now be extended to many-body quantum gases. A natural extension is whether enhanced or diminished work fluctuations result from collective effects, whose nature may be captured under this framework. Since our framework derives from a grand-canonical picture, one expects that fluctuations in work output will be drastically impacted around the critical temperature, resulting from the large density fluctuations, predicted and observed for BECs under a grand-canonical treatment \cite{Schmitt2014,Crisanti2019}. It is also an interesting question whether a similar result is exhibited for an interacting working system. 
It would also interesting to see what effect an interacting BEC has on the work output and dissipation for a cycles that cross the transition.

Using a known power-efficiency trade-off relation we have characterized the performance of the BEC engine through a geometric figure of merit and shown that despite an increased dissipation, the BEC-engine can produce a higher power output for a given efficiency when compared to a collection of SPEs. 

Using thermodynamic geometry, our construction provides a systematic and universal method to examine the collective effects of such many-body engine cycles operating in the adiabatic-response regime. It should therefore be straightforward to apply this framework to other working systems in order to analyze the collective effects on engine performance. BECs offer a effect. Interacting systems ...

 It is also an interesting question whether a similar result is exhibited for an interacting working system. 
It would also interesting to see what effect an interacting BEC has on the work output and dissipation for a cycles that cross the transition. 

Such as with the quantum many-body nature of BECs, engines consisting of two level systems exhibit cooperative advantages, owing to their indistinguishably with respect to coupled temperature baths \cite{Niedenzu2018}. Here the system operates between two fixed temperature baths. Whether this can be incorporated into this framework is an open question., where geometric bounds exist for devices operating between fixed temperature baths \cite{Eglinton2022} is an open question.
